Building Efficient Concurrent Graph Object through Composition of List-based Set

In this paper, we propose a generic concurrent directed graph (for shared memory architecture) that is concurrently being updated by threads adding/deleting vertices and edges. The graph is constructed by the composition of the well known concurrent list-based set data-structure from the literature. Our construction is generic, in the sense that it can be used to obtain various progress guarantees, depending on the granularity of the underlying concurrent set implementation - either blocking or non-blocking. We prove that the proposed construction is linearizable by identifying its linearization points. Finally, we compare the performance of all the variants of the concurrent graph data-structure along with its sequential implementation. We observe that our concurrent graph data-structure mimics the performance of the concurrent list based set.

==> acyclicity.tex <==
\section{Maintaining Graph Acyclicity}
\label{sec:Maintaining-Graph-Acyclicity}

\noindent In this section, we consider the problem of maintaining an invariant of acyclicity in this concurrent dynamic graph data structure. As described earlier, the objective is to maintain an acyclic conflict graph of transactions for \sgt. For a concurrent graph to be acyclic, the graph should maintain the acyclic property at the end of each operation in the equivalent sequential history. To achieve this, we try to ensure that the graph stays acyclic in all the global states. 

It is easy to see that a cycle can be created only on addition of edge to the graph. We modify the concurrent graph data structure presented in the earlier section to support this acyclic property. The sequential specification of $\acadde$ is relaxed as follows: after a new directed edge has been added to the graph (in the shared memory), we verify if the resulting graph is acyclic. If it is, we leave the edge. Otherwise we delete the edge from the shared memory. Thus $\acadde(u, v)$ may fail even if the edge $(u, v)$ was not already part of the graph. The sequential specification of the graph data structure with acyclic property is same as that of sequential specification of graph data structure as shown in the Table \ref{tab:seq-spe}, except $\adde$ $\mth$. This modified specification is shown in the Table \ref{tab:seq-spe-acyclic}.


\begin{table*}[th]
\centering
%\scriptsize
\begin{tabular}{ m{6cm}| m{6cm} } 
%\label{struct:vertex-edge}
 \hline
  %\hf{Edge Structure} &  \hf{Vertex Structure} \\ 
  {Edge Node} &  {Vertex Node} \\ %[-2ex]
   & \\[-2ex]
   \hrule & \hrule\\[-2ex]
    \begin{verbatim}
class enode{
  int val;
  enode enext;
  enum status = {transit,
            marked, added};
  Lock lock;
  enode(int key){  
     val = key;
     status = transit;
     enext = null;
     lock = new Lock();
    }
};
\end{verbatim}
    &
\begin{verbatim}
class vnode{
    int val;
    vnode vnext;
    enode EdgeHead, EdgeTail;
    boolean marked;
    Lock lock;
    vnode(int key){  
        val = key;
        marked = false;
        vnext = null;
        EdgeHead = new enode(-infinity);
        EdgeTail = new enode(+infinity);        
        EdgeHead.enext = EdgeTail;
        lock = new Lock();
    }
};
\end{verbatim}
\hfill  \\[-2ex]
\hrule & \hrule \\[-2ex]
\end{tabular}
\caption{Structure of Vertex and Edge Node for maintaining Acyclicity.}
\label{tab:struc-cyc}
\end{table*}


%\noindent It is easy to see that a cycle can be created only on addition of edge to the graph. We modify the concurrent graph data structure presented in the earlier section to support this acyclic property. The sequential specification of $\acadde$ is relaxed as follows: after a new directed edge has been added to the graph (in the shared memory), we verify if the resulting graph is acyclic. If it is, we leave the edge. Otherwise we delete the edge from the shared memory. Thus $\acadde(u, v)$ may fail even if the edge $(u, v)$ was not already part of the graph.\\[0.1cm]

%constructed after the linearization of the concurrent history. We present an algorithm for concurrent cycle detection based on reachability. 

%\vspace{-1.8cm}
%-----------moved from section 4----------
 %If this method returns $true$, then the graph acyclic property maybe violated. To identify this, the method invokes $CycleDetect$. In section 5, we provide two solution approaches for cycle detection in the concurrent graph environment. At any instant, when a new directed edge is added to the graph, the concurrent graph is checked for maintaining acyclicity. If it does not preserve, then the edge is removed.
%-------------------------------------------------------------




%\vspace{-3cm}
%\noindent Table \ref{tab:struc-cyc} describes the modified fields of the edge and vertex nodes of the Table \ref{tab:struct:vertex-edge}. When a new edge node is added, its \emph{status} is initially set to \emph{transit}. The overall idea is that it is allowed to be logically added to the graph i.e. its status set to \emph{added} only after it is ensured that the edge has not formed any cycle. Thus, we ensure that in any global state all the edges in `added' state do not form a cycle. An edge node in transit state can not get removed by any other concurrent thread. However, every thread performing a cycle detect on the concurrent graph can see all edges in $transit$ as well as $added$ state. \\[0.1cm] 

%\noindent The sequential specification of the graph data structure with acyclic property is same as that of sequential specification of graph data structure as shown in the Table \ref{tab:seq-spe}, except $\adde$ $\mth$. This modified specification is shown in the Table \ref{tab:seq-spe-acyclic}.

\begin{table*}[th]
 \centering
  \captionof{table}{Sequential Specification of the Graph Data Structure with Acyclic property } \label{tab:seq-spe-acyclic} 
\begin{tabular}{ |m{3.5cm}|m{1cm}|m{4.5cm}|m{4.5cm}| } 

\hline
  \textbf{Method} & \textbf{Return Value} & \textbf{Pre-state}($S$: global state)  & \textbf{Post-state}( $S'$: future state of $S$ such that $S \sqsubset S'$)  \\ 
  
  
	\hline 
	$\acadde (u, v)$  & $true$ &$ S: \langle u,v \in S.\abgv \wedge  ((u,v) \in S.\abge \vee (u,v) \notin S.\abge) \wedge (\abg \text{ is Acyclic)}  \rangle$ & $ S':\langle (u,v) \in S'.\abgv \wedge (u,v) \in S'.\abge \wedge (\abg \text{ is Acyclic)} \rangle$	 \\
	\hline 
	$\acadde(u, v)$  & $false$ &$ S: \langle  u \notin S.\abgv \vee v \notin S.\abgv \wedge (\abg \text{ is Acyclic)} \rangle$ & Same as pre-state \\%$\forall S: ((u,v) \notin S.S(E).AbG)  \vee (u \notin S.\abgv) \vee (v \notin S.\abgv)$ 
	\hline 
 
\end{tabular}
\end{table*}
%----------------------------------------------------

%--------------------------------------------------------------------------------------------------

Table \ref{tab:struc-cyc} describes the modified fields of the edge and vertex nodes of the Table \ref{tab:struct:vertex-edge}. Each node has a \emph{status} field which can be in one of the three states: \emph{transit, marked, added}. When a new edge node is added, its \emph{status} is initially set to \emph{transit}. The overall idea is that it is allowed to be logically added to the graph i.e. its status set to \emph{added} only after it is ensured that the edge does not form any cycle. Thus, we ensure that in any global state all the edges in `\emph{added}' state do not form a cycle. Although, it is possible that the edges with status \emph{added} and \emph{transit} form a cycle in some global state. 

A thread adds an edge to the graph in \emph{transit} state. If the new \emph{transit} edge does not cause a cycle, then its status is changed to \emph{added}. Otherwise, the new edge is deleted by setting its status to \emph{marked}. An edge node in \emph{transit} state can not get removed by any other concurrent thread. However, every thread performing a cycle detect on the concurrent graph can see all edges in $transit$ as well as $added$ state. 

A side-effect to be observed here is that this may allow \textit{false positives}. This means that the algorithm may detect a cycle even though the graph does not contain one. This can happen in the following scenario; two threads $T_1$ and $T_2$ are adding edges lying in the path of a single cycle. In this case, both threads detect that the newly added edge (in $transit$) has led to formation of a cycle and both may delete their respective edges. However, in a sequential execution, only one of the edges will be removed. We allow this as the resulting graph at the end of each operation is acyclic. From the perspective of application \sgt which uses the graph acyclicity, a false positive implies unnecessary abort of a transaction. But this does not violate the correctness , i.e., serializability in Databases and Opacity in STMs. On the other hand, having a cycle in the application violates correctness and thus should not be allowed. 
%\ref{alg:add:Edge:cd}, \ref{alg:remove:Edge:cd} and \ref{contains:Edge:cd}

Thus to incorporate these changes to preserve acyclicity, the methods exported by the algorithm are modified as: $\acadde$, $\acreme$, $\accone$. Algorithms \ref{validate:Edge:cd}\text{-}\ref{contains:Edge:cd} illustrate these methods. The methods $ValidateVertex$, $\addv$, $\remv$ and $\conv$ remain same as described in Algorithms \ref{validate:Vertex}, \ref{alg:add:Vertex}, \ref{alg:remove:Vertex} and \ref{contains:Vertex} respectively.


\subsection{Working of Concurrent Graph Methods preserving Acyclicity}
\label{sec:working-con-graph-methods-Acyclicity}
\vspace{-1mm}
In this section, we describe the implementation of the concurrent graph structure with acyclicity properties and the working of the various \mth{s}. For a concurrent graph to be acyclic, the graph should maintain the acyclic property at the end of each operation in the equivalent sequential history. Like \cgds the fields in the acyclic structure also declared as atomic. This ensures that operations on these variables happen atomically. In the context of a particular application, the node structure can be easily modified to carry useful data (like weights etc). \\[0.1mm]
\begin{algorithm}[!htb]
	\captionsetup{font=scriptsize}
	\caption{\acvlde Method: Takes two $\enode$ $e_1, e_2$ and validates for presence in the edge list. }
	\label{validate:Edge:cd}
	\begin{algorithmic}[1]
		\scriptsize
		\algrestore{cone}
		\Procedure{\acvlde($e_1\downarrow, e_2\downarrow, flag\uparrow$)}{}
		%        \While {$(read(n_1.status) = transit \vee read(n_2.status) = transit)$}
		%        \EndWhile
 		\If {$(read(e_1.status) = added) \wedge (read(e_2.status) = added) \wedge (read(e_1.enext) = e_2)$} \label{lin:valec2}
		\State {$flag \gets true;$}\label{lin:valec5} {\hspace{.35cm}//validation successful}
		\Else 
		\State {$flag \gets false;$}\label{lin:valec8} {\hspace{.35cm}// validation failed}
		\EndIf
		\State $return;$  {\hspace{.35cm}//return flag}
		\EndProcedure
		\algstore{valec}
	\end{algorithmic}
\end{algorithm}
%------------------------------------------------------------------------------
%\setlength{\textfloatsep}{0pt}
\begin{algorithm}[!htb]
	%\scriptsize
	\captionsetup{font=scriptsize}
	\caption{Modified ValidateEdge Method: Takes two $ENode$ $e_1, e_2$ and validates for presence in edge list.}
		\label{modified-val:Edge}
	\begin{algorithmic}[1]
		\algrestore{valec}
		\scriptsize
		\Procedure{$\modvlde(e_1\downarrow, e_2\downarrow, flag\uparrow$)}{}
		%	\State{// check $e_1$ \& $e_2$ are not marked and $e_1.enext = e_2$.}
		\If {$(read(e_1.status) \neq marked)$ $\wedge$ $(read(e_2.status) \neq marked)$  $\wedge$ $(read(e_1.enext) = e_2$)} \label{lin: modified-val}
		\State {$flag \gets true;$}  \hspace{.5cm}{// validation successful} \label{lin:modvldedge}
		%\State $return;$  \label{lin:vale3.1}
		\Else 
		\State {$flag \gets false;$}  \hspace{.5cm} {//validation fails} 
		%\State $return$;\label{lin:vale5.1}
		\EndIf
		\State {$return$;} \hspace{.5cm} {//return flag}
		\EndProcedure
		\algstore{vale}
	\end{algorithmic}
\end{algorithm}


\begin{algorithm}[!htb]
	\captionsetup{font=scriptsize}
	\caption{AcyclicLocateEdge Method: Takes two keys, $key_1$ and $key_2$, as input and returns the pair of adjacent $\enode$ $\langle e_1, e_2 \rangle$. If $\vnode$ $v_1$ or $v_2$ or $\enode$ $e_2$ is not present, it returns false. Initially enodes $e_1, e_2$ are set to $null$ and $flag$ is set to $true$.}
	\label{locate:Edge-acy}
	\begin{algorithmic}[1]
		\scriptsize
		\algrestore{vale}
		\Procedure{AcyclicLocateEdge ($key_1 \downarrow, key_2\downarrow, val\downarrow, v_1\uparrow, v_2\uparrow, e_1\uparrow, e_2\uparrow, flag\uparrow$)}{}
		\State{$ HelpSearchEdge (key_1 \downarrow, key_2\downarrow, v_1\uparrow, v_2\uparrow, flag \uparrow$);} \label{lin:alocedge}
		\If {($flag$ = $false$)} \label{lin:alocedge-flag}
		\State {$return$; }\hspace{.4cm} { // $v_1$ or $v_2$ not found, returns flag} \label{lin:alocedge-flag-false}
		\EndIf
		\State{/*This lines ensures both the vertices $v_1$ \& $v_2$ have been added to the system by this time  and are not marked*/}
		\If {$(read(v_1.marked)$ $\vee$ $read(v_2.marked))$}  \label{lin:alocedge-marked}
		\State {$flag \gets false$;} 
		\State {$return$; }
		\EndIf
		
		\State{/* Helping for search edge, is a supporting method for locate edge. It locates the vertices $v_1$ \& $v_2$*/}
		\While{(true)} \label{lin:alocedge-help}
		
		\State {$e_1 \gets read(v_1.enext)$;} \label{lin:loce17.0}
		\State {$e_2 \gets read(e_1.enext)$;}\label{lin:loce18.0}
		\State{ /* Search $\enode(key_2)$ without acquiring any locks*/}
		\While{$(read(e_2.val) < key_2)$}\label{lin:loce19.0}
		\State {$e_1 \gets e_2$;} \label{lin:loce20.0}
		\State {$e_2 \gets read(e_2.enext)$;} \label{lin:loce21.0}
		\EndWhile  \label{lin:loce21.01}
		\State {$lock.acquire(e_1)$;}\label{lin:loce23.0}
		\State {$lock.acquire(e_2)$;}\label{lin:loce24.0}
		\If{(val)}  \label{lin:alocedge-val}
		\If{($ModifiedValidateEdge(e_1 \downarrow, e_2 \downarrow, flag \uparrow$))}\label{lin:loce25.0}
		\State{$return;$} \label{line:modf-valid}
		\Else
		\State {$lock.release(e_1)$;}\label{lin:loce28:1.0}
		\State {$lock.release(e_2)$;}\label{lin:loce29:1.0}
		\EndIf
		\ElsIf{($\neg$val)}
		\If{($AcyclicValidateEdge(e_1 \downarrow, e_2 \downarrow, flag \uparrow$))}     \label{lin:acvldedge}
				\State{$return$}; 
			\Else
				\State {$lock.release(e_1)$;}\label{lin:loce28:1.2}
				\State {$lock.release(e_2)$;}\label{lin:loce29:1.2}
			\EndIf
       \Else		
			\State {$lock.release(e_1)$;}\label{lin:loce28:2}
			\State {$lock.release(e_2)$;}\label{lin:loce29:2}
		\EndIf
		\EndWhile \label{lin:alocedge-end}
		\EndProcedure
		\algstore{loce1}
	\end{algorithmic}
\end{algorithm}
%\vspace{-2mm}
\noindent \textbf{\emph{Update Vertex Methods}: - \acaddv \& \acremv} \\
\label{sec:working-con-graph-methods:addv-Acyclicity}
The working of the $\acaddv$ and $\acremv$ methods are similar to the \addv and \remv methods of the \cgds described in the Section \ref{sec:working-con-graph-methods-Acyclicity}. \\ [0.3mm]
\noindent \textbf{\emph{Update Edge Method}:- \acadde }\\
\label{sec:working-con-graph-methods:adde-Acyclicity}
\noindent When a thread wants to add an edge $(u,v)$ to the concurrent graph, it invokes the \emph{AcyclicLocateEdge} method in the Line \ref{lin:addec2}. This \emph{AcyclicLocateEdge} internally invokes the \emph{HelpSearchEdge} method in the Line \ref{lin:alocedge}. The \emph{HelpSearchEdge} described in the Algorithm \ref{helpsearch:Edge}. This method checks for the presence of vertices $u$ and $v$ in the vertex list of the graph. Now we add an additional check to verify that the two vertices are reachable from the \vh in Line \ref{lin:alocedge-marked}. The reason for this is as explained in Figure 1. Once the vertices have been found, the thread traverses the edge list of vertex $u$ until an edge node with key greater than $v$ has been encountered, say $ecurr$ and it's predecessor say $epred$. The thread does all this without acquiring locks. It then acquires locks on both $epred$ and $ecurr$ and performs validation by invoking \emph{\modvlde} in the Line \ref{lin:loce25.0}. The \emph{\modvlde} is described in the Algorithm \ref{modified-val:Edge}. This method checks that the locked nodes have not been deleted and are reachable. In other words, it successfully validates even though the nodes are in \textit{transit} state and returns the locked nodes. In case the validation fails, it releases the locks and retries. Once the $epred$ and $ecurr$ edge nodes have been found, a new edge node (with status as $transit$) is added between them, if the key does not already exists. After this the acquired locks are released. If the node was newly added, then it invokes the \emph{PathExists} method in the Line \ref{lin:addedge:cycle} to check if there exists a path from vertex $v$ to $u$. The \emph{PathExists} method is described in the Algorithm \ref{algo:pathexists}.\\
%It creates a local $ReachSet$ of all vertices reachable from $v$, with an $explored$ boolean field corresponding to each vertex in this set. It traverse the adjacency list of $v$ to find $u$ in the concurrent graph, without acquiring locks. All these traversed vertices edge nodes are added to the local $ReachSet$ in Line \ref{lin:path-loc-reach} and the vertex $v$ is marked to be $explored$ in the Line \ref{lin:path-explored}. From the Line \ref{lin:wait-free:while:explore}- \ref{lin:path-explored-end} it recursively visits the outgoing edges which are not marked from the neighbours of $v$ to find $u$ . This is done until all the vertices in all the paths from $v$ to $u$ and have been $explored$ or a cycle has been detected.  \\
\noindent Now, if there exists a path from $v$ to $u$, it means a cycle has been detected, then the edge $(u, v)$ must be removed by setting its status to \emph{marked}, else it must be changed to \emph{added}. However, for deletion of the node in transit, we must be able to get the pointer to the predecessor node. Hence it invokes the \emph{\newloce} in the Line \ref{lin:newloce-test}. It is to be noted that during this phase, the vertex $u$ could have been deleted. Hence \emph{\newloce} method starts scans directly the \elist of the $u$ until it finds a \enode with a key value greater than or equal to $e_3.key$ and it's predecessor say $epred$. After this, validation is performed by invoking the \emph{\modvlde} method in the Line \ref{lin:modvlde-invoke} to check if the locked edge nodes are reachable and unmarked. If the validation is successful, the new edge node $e_3$ is removed by making \emph{status} to \emph{marked} in the Line \ref{lin:status-addec14}. If there is no path from $v$ to $u$, means cycle has not been detected, so the status of the $e_3$ is simply changed to \emph{added} in the Line{lin:addec14}. The \emph{AcyclicAddEdge} method is described in Algorithm \ref{alg:add:Edge:cd}.\\[0.2mm]

%-------------------------------------------------
\begin{algorithm}[!htb]
	\captionsetup{font=scriptsize}
	\caption{New LocateEdge Method: Takes two keys, $key_1$ and $key_2$, as input and returns the pair of adjacent $\enode$ $\langle e_1, e_2 \rangle$. If $\vnode$ $v_1$ or $v_2$ or $\enode$ $e_2$ is not present, it returns false. Initially enodes $e_1, e_2$ are set to $null$ and $flag$ is set to $true$.}
	\label{newlocate:Edge}
	\begin{algorithmic}[1]
		\scriptsize
		\algrestore{loce1}
		\Procedure{\newloce ($key_1 \downarrow, key_2\downarrow, v_1\downarrow, v_2\downarrow, e_1\uparrow, e_2\uparrow, flag\uparrow$)}{}
		%    \State{$ HelpSearchEdge (key_1 \downarrow, key_2\downarrow, v_1\uparrow, v_2\uparrow, flag \uparrow$);}
		%   \If {($flag$ = $false$)}
		%   \State {$return$; }\hspace{.4cm} { // $v_1$ or $v_2$ not found, returns flag}
		%   \EndIf
		%   \If {$(read(v_1.marked)$ $\vee$ $read(v_2.marked))$}
		%   \label{lin:nloce8:16}
		%   \State {$flag \gets false$;} 
		%   \State {$return$; }
		%   \EndIf
		\While{(true)}
		%	\State{/* Helping for search edge, is a supporting method for locate edge. It locates the vertices $v_1$ \& $v_2$*/}
		\State {$e_1 \gets read(v_1.enext)$;} 
		\State {$e_2 \gets read(e_1.enext)$;}
		\State{ /* Search $\enode(key_2)$ without acquiring any locks*/}
		\While{$(read(e_2.val) < key_2)$}
		\State {$e_1 \gets e_2$;} 
		\State {$e_2 \gets read(e_2.enext)$;} 
		\EndWhile
		\State {$lock.acquire(e_1)$;}
		\State {$lock.acquire(e_2)$;}
		\If{($\modvlde(e_1 \downarrow, e_2 \downarrow, flag \uparrow$))} \label{lin:modvlde-invoke}
		%\State{$flag \gets true$}; 
		\State return; \hspace{.4cm} {// returns true if validation succeeds.}
		\Else 
		\State {$lock.release(e_1)$;}
		\State {$lock.release(e_2)$;} \hspace{.4cm} {// validation failed, try again}
		\EndIf
		\EndWhile
		\EndProcedure
		\algstore{loce2}
	\end{algorithmic}
\end{algorithm}
%-------------------------------------------------

\begin{algorithm}[!htb]
	\captionsetup{font=scriptsize}
	\caption{\acadde Method: $\enode(key_2)$ gets added to the edge list of $\vnode(key_1)$, if it is not already part of it and does not form a cycle. Initially $flag$ is set to $true$.}
	\label{alg:add:Edge:cd}
	\begin{algorithmic}[1]
		\scriptsize
		\algrestore{loce2}
		\Procedure{\acadde ($key_1\downarrow$,$key_2\downarrow, flag\uparrow$)}{}
		\State {$ AcyclicLocateEdge(key_1\downarrow, key_2\downarrow, true\downarrow, v_1\uparrow, v_2\uparrow, e_1\uparrow, e_2\uparrow, flag\uparrow)$}  { // Algorithm \ref{locate:Edge-acy}}  \label{lin:addec2}
		\State{/*$\vnode(key_1)$ or $\vnode(key_2)$ not found*/}
		\If {($flag$ = $false$)} \label{lin:acadde-flag}
		\State {$return$;} 
		\EndIf
		\If {$(read(e_2.val) \neq key_2$)} \label{lin:addec2.1} \label{lin:addec3}  {\hspace{.2cm}//$\enode(key_2)$ not present}
		\State{/*$e_3.status$ is set to $transit$ initially*/}
		\State {$write(e_3$, $new$ $\enode(key_2))$;}  \label{lin:addec4}
		\State {$write(e_3.enext, e_2)$;} \label{lin:addec5}
		\State {$write(e_1.enext, e_3)$;} \label{lin:addec6}
		\State {$lock.release(e_1)$;} 
		\State {$lock.release(e_2)$;}
		%\State {goto Line \ref{lin:addedge:cycle};} \label{lin:adde9}
		\Else
		%		\State {$flag \gets false$}  
		\State {$lock.release(e_1)$;} \label{lin:addec11} {\hspace{.25cm}// $\enode(key_2)$ already present}
		\State {$lock.release(e_2)$;} \label{lin:addec12}
		\State {$return;$ } \label{lin:addec13.0}
		\EndIf
		\State $cycle\_flag \gets PathExists$($key_2\downarrow$, $key_1\downarrow$); \label{lin:addedge:cycle} {\hspace{.25cm} //check for cycle}

		\If {$(cycle\_flag = true$)}\label{lin:addec13}  {\hspace{.25cm}//cycle detected}
		\State {$ \newloce(key_1\downarrow, key_2\downarrow, v_1\downarrow, v_2\downarrow, ne_1\uparrow, ne_2\uparrow, flag\uparrow)$} {// Algorithm \ref{newlocate:Edge}} \label{lin:newloce-test}
		\State $write(e_3.status, marked);$ \label{lin:status-addec14}  {\hspace{.25cm} //logical removal}
		\State $write(ne_1.enext, e_2);$      
		\State {$flag \gets false;$}\label{lin:addec15}
		\State {$lock.release(e_1)$;} \label{lin:adde71}
		\State {$lock.release(e_2)$;} \label{lin:adde81}
		\Else
		\State $write(e_3.status, added);$\label{lin:addec14}  {\hspace{.25cm}//logical addition}
		%        \State {$flag \gets true;$}\label{lin:addec14}
		\EndIf
		
		\State {$return;$  \hspace{.25cm} // return flag}
		\EndProcedure
		\algstore{addec}
	\end{algorithmic}
\end{algorithm}
%-------------------------------------------------

\noindent\textbf{\emph{Update Edge Method}:- \acreme}\\
\label{sec:working-con-graph-methods:reme-Acyclicity}
\begin{algorithm}[!htb]
	\captionsetup{font=scriptsize}
	\caption{\acreme Method: $\enode(key_2)$ gets removed from the edge list of $\vnode(key_1)$, if it is part of it.  }
	\label{alg:remove:Edge:cd}
	\begin{algorithmic}[1]
		\scriptsize
		\algrestore{addec}
		\Procedure{\acreme ($key_1\downarrow$, $key_2\downarrow, flag\uparrow$)}{}
		\State{$ AcyclicLocateEdge(key_1\downarrow, key_2\downarrow, false\downarrow, v_1\uparrow, v_2\uparrow, e_1\uparrow, e_2\uparrow, flag\uparrow);$}   \label{lin:remec2}
		{ // Algorithm \ref{locate:Edge-acy}}
		\State{/* $\vnode(key_1)$ or $\vnode(key_2)$ not found*/}
		\If {($flag$ = $false$)}  \label{lin:remec-flag}
		\State {$return$;}        
		\EndIf
		\If {$(read(e_2.val) = key_2)$} \label{lin:remec3}
		\State {$write(e_2.status, marked)$;} \label{lin:remec4}  {\hspace{.3cm}//logical removal}
		\State {$write(e_1.enext, e_2.enext)$;} \label{lin:remec5}
		%  \State {$flag \gets true;$}  \label{lin:reme12}
		%\State {return $true$;} \label{lin:reme8}
		\EndIf \hspace{.35cm}  { // not present}
		\State {$lock.release(e_1)$;} \label{lin:remec10}
		\State {$lock.release(e_2)$;} \label{lin:remec11}
		%	 \State {$flag \gets true;$}  \label{lin:remec12}
		%\State $return$;\label{lin:remec12.1}
		%\EndIf
		\State {$return$;} \hspace{.35cm} {// return flag}
		
		\EndProcedure
		\algstore{remec}
	\end{algorithmic}
\end{algorithm}
%-------------------------------------------------
\noindent In $\acreme(u,v)$, the $\enode$ $v$ is removed from $u$'s \elist. It starts by invoking \emph{AcyclicLocateEdge} method in the Line \ref{lin:remec2}. This is same as described in the \emph{AcyclicAddEdge} above, with the only difference that it performs validation by invoking \emph{AcyclicValidateEdge} in Line \ref{lin:acvldedge}. The role of this method is to check if the locked edge nodes are \emph{added} in the \cgds. This is important since transit edge nodes cannot be deleted. If the edge node to be deleted is already present then deletion of \enode $v$ takes in two phases: first logical removal of the \enode $v$ by setting the status field in the Line \ref{lin:remec4} to \emph{marked}. Then, \enode $v$ is removed physically from $u$'s \elist by changing the pointers in the Line \ref{lin:remec5}. The \emph{AcyclicRemoveEdge} method is described in Algorithm \ref{alg:remove:Edge:cd}.\\[0.2mm]

\noindent\textbf{\emph{Read-only Methods}: - \acconv \& \accone}\\
\begin{algorithm}[!htb]
	\captionsetup{font=scriptsize}
	\caption{\accone Method: Returns $true$ if $\enode(key_2)$ is part of the edge list of $\vnode(key_1)$ and returns $false$ otherwise. }
	\label{contains:Edge:cd}
	\begin{algorithmic}[1]
		\scriptsize
		\algrestore{remec}
		\Procedure{\accone ($key_1\downarrow$, $key_2\downarrow, flag\uparrow$)}{}
		\State{$ HelpSearchEdge (key_1 \downarrow, key_2\downarrow, v_1\uparrow, v_2\uparrow, flag \uparrow$);} {//Algorithm \ref{helpsearch:Edge}} \label{helpsearch:Edge-inaccone}
		\State{/* $\vnode(key_1)$ or $\vnode(key_2)$ not found */}
		\If {$(flag$ = $false$)} \label{lin:conec-flag-sta}
		\State{$return$;} \label{lin:conec-flag-false}
		\EndIf
		\State {$e \gets read(v_1.enext)$;}\label{lin:conec16}
		\While{$(read(e.val) < key_2)$} \label{lin:conec17}
		\State {$e \gets read(e.enext)$;} \label{lin:conec18}
		\EndWhile \label{lin:conec17.1}
		%  \State{$return$ $(read(e.val)$ = $key$ \&\& $(read(e.status) = added))$;}
		%\label{lin:cont-tf:Edge} 
		%\label{lin:cone20}
		\If {$(read(e.val) \neq key) \vee (read(e.status) \neq added)$} 
		\State {$flag \gets false;$}\label{lin:remec8}
		%\Else
		\Else
		\State {$flag \gets true;$}\label{lin:conec23}
		%    \State $return;$ \label{lin:conec23.1}
		\EndIf
		\State {$return$;} 
		\EndProcedure
		\algstore{conec}
	\end{algorithmic}
\end{algorithm}
The $\acconv(u)$ method works similar to the wait-free \conv of method described in the Algorithm \ref{contains:Vertex}. It proceeds by scanning the \vlist, without acquiring any locks until it encounters a \vnode of key greater than or equal to $u$. It returns $true$ if the \vnode it was searching for is present and unmarked in the graph and otherwise returns $false$. \\
\noindent Similarly, the $\accone(u, v)$ method first scans the \vlist like \conv for each vertex $u$ and $v$ and checks both the vertices are present and unmarked. It traverse the \elist without acquiring any locks on \enode. It returns $true$ if the \enode it was searching for is present and it's status is \emph{added} in the \elist of \vnode $u$ and otherwise returns $false$. The \accone method is described in the Algorithm \ref{contains:Edge:cd}.








\begin{algorithm}[!htb]
	\captionsetup{font=scriptsize}
	\caption{Wait-Free Reachability $PathExists$ Method: Returns $true$ if there exists a path from $\vnode(key_1)$ to $\vnode(key_2)$ and returns $false$ otherwise.}
	\label{algo:pathexists}
	\begin{algorithmic}[1]
		\scriptsize
		\algrestore{conec}
		\Procedure{PathExists($key_1\downarrow, key_2\downarrow, flag\uparrow$)}{}
		\State {Set $local\_R$ $\leftarrow$ $\phi$} \Comment{Set does not allow duplicates }
		\State {$ v_1 \gets read(\vh)$;} 
		\While {($read(v_1.val) < key_1$)} 
		\State {$v_1 \gets read(v_1.vnext)$;}
		\EndWhile
		\If {$(read(v_1.val) \neq key_1 \vee read(v_1.marked))$}
		\State {$flag \gets false$;}
		\State {$return;$} %/*path does not exist from keyu to keyv*/
		\EndIf
		\State{$e_1 \gets read(v_1.enext)$;}
		\While{$(read(e_1.enext) \neq null)$}
		\If{($ read(e_1.marked = false ) $)}
		\State {$local\_R \gets local\_R \cup read(e_1.val)$; }
		\EndIf
		\State{$e_1 \gets read(e_1.enext)$;}
		\EndWhile
		
		\If{($key_2 \in local\_R$)} 
		\State {$flag \gets true$;}
		\State {$return;$} %/*path does not exist from keyu to keyv*/
		\EndIf
		\State { $key_1.explored \gets true$;} \Comment{ as explored in local copy}
		\While{($\exists key_x \in local\_R $ $|$ $(key_x.explored = false )$}  \label{lin:wait-free:while:explore}
		\State{$v_2 \gets read(\vh)$;}
		\While{($ read(v_2.val) < key_x$)}
		\State {$v_2 \gets read(v_2.vnext)$;}
		\EndWhile
		\If{($read(v_2.val) \neq key_x \vee read(v_2.marked)$)}
		\State {$key_x.explored \gets true$;}
		\State $continue: Line \ref{lin:wait-free:while:explore}$;
		\EndIf
		\State {$e_2 \gets read(v_2.enext)$;}
		\While{($ read(e_2.enext) \neq null$)}
		\If{($ read(e_2.marked) = false $)}
		\State {$local\_R \gets local\_R \cup read(e_2.val)$; } \label{lin:path-loc-reach}
		\EndIf
		\State {$e_2 \gets read(e_2.enext)$;}
		\EndWhile
		\If{($key_2 \in local\_R$)} 
		\State {$flag \gets true$;}
		\State {$return;$} %/*path does not exist from keyu to keyv*/
		\EndIf
		\State {$key_x.explored \gets true$;} \label{lin:path-explored}
		\EndWhile \label{lin:path-explored-end}
		\State {$flag \gets false$;}
		\State {$return;$} %/*path does not exist from keyu to keyv*/
		\EndProcedure
		% \algstore{wfrc}
	\end{algorithmic}
\end{algorithm}

\subsection{Wait-Free Reachability} 
\noindent The following subsection presents an algorithm based on reachability for ensuring acyclicity in the concurrent graph developed. Given a directed graph, $G = (V, E)$ and two vertices $u, v \in V$, a vertex $v$ is reachable from another vertex $u$, if there exists a path from the vertex $u$ to $v$ in $G$. By using this idea of reachability, we define a method for cycle detection in concurrent directed graphs. Before invoking this method, we must remember that $\acadde(x,y)$ has already returned $true$. So this is to check if there exists a path from vertex $y$ to $x$ in the concurrent graph. The $reachability$ method creates a local $ReachSet$ of all vertices reachable from $y$, with an $explored$ boolean field corresponding to each vertex in this set. The reachability method begins by traversing the adjacency list of $y$ to find $x$ in the concurrent graph, without acquiring locks. All these traversed vertices edge nodes are added to the local $ReachSet$ and the vertex $y$ is marked to be $explored$. Now, the method recursively visits (similar to breadth first traversal, BFS) the outgoing edges (which are not marked) from the neighbours of $y$ to find $x$. Clearly, this is done until all the vertices in all the paths from $y$ to $x$ in $G$ have been $explored$ or a cycle has been detected in the graph. This method is described in Algorithm \ref{algo:pathexists}.

However, in the concurrent setting, the set of vertices in the path keep varying dynamically. Since the key size is finite and all keys are unique, the adjacency list will be traversed in finite number of steps. Also, since there can only be a finite number of vertices in the path from $v$ to $u$, this method will terminate in a finite number of steps. We define $reachability$ without acquiring any locks and it terminates in a finite number of steps, so it satisfies \textit{wait-freedom} guarantee. 

Once a cycle has been detected, then the edge which caused the cycle is removed from the concurrent graph (by invoking \reme) else the algorithm proceeds normally. An execution of the algorithm is illustrated in Figure \ref{fig:WFR}.

%---------------------------
\begin{figure}[ht]
   \centering
   \centerline{\scalebox{0.6}{\input{figs/WFR.pdf_t}}}
   \caption{An execution of wait-free reachability for concurrent cycle detect. Figure (a) is the initial graph when a thread $T_1$ is trying to concurrently $\acadde(3,7)$ to the graph. Figure (b) depicts the graph when thread $T_1$ has finished adding edge $(3,7)$ and is invoking $PathExists$. Concurrently, thread $T_2$ is trying to $\acadde(4, 7)$. Figure (c) shows the reachability path from vertex $7$ to $3$ as computed by thread $T_1$. A cycle has now been detected and hence the edge $(3,7)$ will now be removed. Similarly, the thread adding edge $(4,7)$ will also invoke $PathExists$ afterwards and remove it.}
   \label{fig:WFR}
\end{figure}
%\vspace{-0.4cm}

\subsection{Correctness: Linearization Points}
\vspace{-2.5mm}
In this subsection, we define the $Linearization$ $Points(LP)$ of methods of the concurrent graph data structure with acyclicity. Only the $LP$ of $\acadde(u, v)$ changes due to the introduction of acyclic invariant.

We linearize a successful $\acadde(u,v)$ method call within its execution interval at the earlier of the following points; (1) if there is no successful concurrent $\remv$ on $u$ and $v$, the $LP$ is defined as the last of $read(e_2.val)$ in Line \ref{lin:addec3} and $write(e_3.status, added)$ in Line \ref{lin:addec14}, depending upon execution. If the last line to execute is \ref{lin:addec3}, the edge $(u,v)$ is already present in the edge list of the vertex $u$ and  whereas Line \ref{lin:addec14} implies that the edge $(u,v)$ is not present earlier and this line adds a new edge node $(u,v)$ such that it is now reachable from $\vh$ of the vertex list; (2) if there is a successful concurrent $\remv$ on $u$ or $v$ or both, the $LP$ is the point immediately before the first $LP$ of successful concurrent delete on vertex $u$ or $v$. 

For an unsuccessful $\acadde(u,v)$ call, the $LP$ is defined to be within its execution interval at the earlier of the following points; (1) if there is no successful concurrent $\addv$ on $u$ and $v$, the $LP$ is last of $read(u.val)$ in Line \ref{lin:helploce8}/\ref{lin:helploce8.1}  where $u$ is not found in vertex list or $read(u.marked)$ in Line \ref{lin:helploce8}/\ref{lin:helploce8.1}  where $u$ is found to be marked or $read(v.val)$ in Line \ref{lin:helploce16}/\ref{lin:helploce16.1}  where $v$ is not found in the vertex list or $read(v_2.marked)$ in Line \ref{lin:helploce16}/\ref{lin:helploce16.1}  where $v$ is found to be marked or $write(e_3.status, marked)$ in Line \ref{lin:status-addec14} depending upon the execution; (2) if there is a successful concurrent $\addv$ on $u$ or $v$ or both, it is linearized at the point immediately before the $LP$ of the first successful concurrent $\addv$ on $u$ or $v$. 

%\noindent \textbf{Lemma 3}: In any execution of the reachability algorithm, all the edges of the graph with the state $added$ do not form a cycle.


\subsection{Safety: Proof Outline}
In this subsection, we try to formalise the proof of our concurrent graph data structure with acyclic invariant based on $\lp$ events of the methods. Here we show that the $\acadde$ maintains acyclicity property. The proof of other properties for maintaining sequential consistency (mentioned below) can be shown similar to the proof in \subsecref{ds-proof}. 
\begin{lemma}
	\label{lem:linealizability-acyclic}
	The algorithms employed for our acyclic \cgds are linearizable.
\end{lemma}

\begin{lemma}
	The methods $\addv$, $\remv$, $\acadde$ and \\ $\acreme$ are deadlock-free and $\conv$, $\accone$ and $PathExists$ are wait-free.
\end{lemma}


\noindent Now, we show the proof of graph acyclicity. For simplicity in this proof sketch, we assume that there are no concurrent add vertex and remove edges/vertices as they do not affect acyclicity property.  

\begin{lemma}
\label{lem:uv-path}
Consider a state $S$ in which there is a path from vertex $u$ to $v$. Then if a thread invokes $PathExists(u, v)$ in $S$ and there are no edge deleted in this path between this \mth invocation and response then $PathExists(u, v)$ will return true.
\end{lemma}

\begin{proofsketch}
The proof of this lemma comes directly from the working of the algorithm.
\end{proofsketch}


\begin{lemma}
\label{lem:addE-conc-acyclic}
In any global state $S$, all the edges with the status \emph{added} are acyclic in $S.\abg$. 
\end{lemma}

\begin{proofsketch}
We initially start with an acyclic graph. Let the cycle be formed in $\abg$ after the successful invocation \& return of $\acadde(u, v)$ by a thread $T_i$. This implies that in the post-state of the \lp of $\acadde(u, v)$, say $S'$ there is a cycle consisting of edges with status \emph{added}. From our assumption, $S'$ the first state in which such a cycle exists. Let $S$ be the pre-state of $\acadde(u, v)$. Then in $S.\abg$ there is a path from the $v$ to $u$. 

W.l.o.g, let the path in $S$ consist of the following vertices: $v \xRightarrow{a} n1 \xRightarrow{a} n2 \ldots nk \xRightarrow{a} u$ where $v \xRightarrow{a} n1$ implies that the edge is in status \emph{added}. From our assumption, all these edges are in state \emph{added} in $S$. From the working of the algorithm all these edges must have been added as \emph{transit} earlier. Among these set of edges, let us suppose that the edge $ni \xRightarrow{t} nj$ be the last edge to be added in the state \emph{transit} by a thread $T_x$ (which could be same as $T_i$). Note that this edge need not be the last edge to be converted to the status \emph{added} in this set. 

Let $ni \xrightarrow{t} nj$ and $u \xrightarrow{t} v$ be the events of the corresponding edges getting added to the $\abg$ with status \emph{transit}. Now, we have two cases:

\begin{itemize}
\item $ni \xrightarrow{t} nj  <_E u \xrightarrow{t} v$: Here $ni \xrightarrow{t} nj$ got added before $u \xrightarrow{t} v$. Thus from our assumption after $ni \xrightarrow{t} nj$ has got added, there is a path from $v$ to $u$ in a state $S1$ consisting of edges with status either as \emph{transit} or \emph{added} in the path. As per the algorithm, $T_i$ will invoke $PathExists(v, u)$ after $u \xrightarrow{t} v$. This from \lemref{uv-path}, this \mth would then return true since there is a path from $v$ to $u$. Hence, $T_i$ will convert not the status of the edge from \emph{transit} to \emph{added} and thus deleting this edge directly. Hence this case is not possible.

\item $u \xrightarrow{t} v <_E ni \xrightarrow{t} nj$: Here, $u \xrightarrow{t} v$ has got added before $ni \xrightarrow{t} nj$. Now consider the state $S1$ just after adding of $ni \xrightarrow{t} nj$. In this state from our assumption, we have that $u \xrightarrow{t} v$. Let us consider the connectivity between $nj$ and $ni$. Originally, we had assumed that there is a path from $v$ to $u$ through $ni$ and $nj$ with $ni$ to $nj$ being the last edge added. Thus from our assumption in $S1$, 

\begin{equation}
\label{eq:v-ni}
v \xRightarrow{t/a} ni-1 \xRightarrow{t/a} \ldots ni
\end{equation}

This equation implies that there is a path from $v$ to $ni$ through a series of edges which are in states either \emph{added} or \emph{transit}. Similarly, we have, 

\begin{equation}
\label{eq:nj-u}
nj \xRightarrow{t/a} nj+1 \xRightarrow{t/a} \ldots u
\end{equation}

From the condition of this case, we have that an edge from $u$ to $v$ was added in \emph{transit} state before. From our assumption in $S1$ this edge would still be be \emph{transit}. Thus we have that 

\begin{equation}
\label{eq:u-v}
u \xRightarrow{t} v
\end{equation}

%Combining Equations \ref{eq:v-ni}, \ref{eq:nj-u}, \ref{eq:ni-nj}, \ref{eq:u-v}, we get that there is a path from $nj$ to $ni$ in $S1$. Thus when $T_x$ invokes $PathExists(nj, ni)$ after $S1$, the \mth will return true. This implies that $T_x$ will not change the status of the edge $ni$ to $nj$ as \emph{added}. Hence when $T_i$ changes the status of edge $u$ to $v$ to \emph{added} the path $v$ to $u$ will not exist. Hence a cycle is not possible.

Combining Equations \ref{eq:v-ni}, \ref{eq:nj-u}, \ref{eq:u-v}, we get that there is a path from $nj$ to $ni$ in $S1$. Thus when $T_x$ invokes $PathExists(nj, ni)$ after $S1$, from \lemref{uv-path} we get that this \mth will return true. This implies that $T_x$ will not change the status of the edge $ni$ to $nj$ as \emph{added}. Hence when $T_i$ changes the status of edge $u$ to $v$ to \emph{added} the path $v$ to $u$ will not exist. Hence a cycle is not possible.
\end{itemize}

Thus in both the cases, a cycle is not possible. 

\end{proofsketch}


\begin{lemma}
\label{lem:addET-conc-acyclic}
If some $\acadde(key_1,key_2)$ method returns true in $E^H$, then 
\begin{enumerate}[label=\ref{lem:addET-conc-acyclic}.\arabic*]
    \item \label{lem:addET-conc-acyclic-pre}
    The corresponding vertex nodes, $\vnode(key_1)$ and $\vnode(key_2)$ will be present in the pre-state of \lp event of the method and the graph is acyclic. Formally, $\langle \acadde(key_1,key_2,true) \Longrightarrow (\vnode(key_1) \wedge \vnode(key_2) \in \prees{\acadde(key_1,key_2,true)}) \wedge (\abg \text{ is Acyclic)} \rangle$. 
\item \label{lem:addET-conc-acyclic-post}
    The corresponding vertex nodes, $\vnode(key_1)$ and $\vnode(key_2)$ will be present in the post-state of \lp event of the method and the graph is acyclic. Formally, $\langle \acadde(key_1,key_2,true) \Longrightarrow (\vnode(key_1) \wedge \vnode(key_2) \in \postes{\acadde(key_1,key_2,true)}) \wedge (\abg \text{ is Acyclic)} \rangle$. 
\end{enumerate}    
\end{lemma}

\begin{proofsketch}
\begin{itemize}
\item \textbf{\ref{lem:addET-conc-acyclic-pre}}:
\begin{enumerate}
\item No successful concurrent $\remv$ on $key_1$ \& $key_2$: By observing the code, we realise that $HelpSearchEdge$ returns successfully only when $\vnode(key_1)$ \& $\vnode(key_2)$ were found to be present in the vertex list at least in one state of the execution. Now after this, the vertex nodes are again tested for removal. Thus, we can conclude that in the post-state of Line \ref{lin:loce8:16}, vertex nodes $\vnode(key_1)$ and $\vnode(key_2)$ must belong to $S.\abgv$. Since there is no concurrent deletion of these vertices, we conclude that both the vertex nodes are present in the pre-state of $\lp$ of this method. And from the Lemma \ref{lem:acyclic}, the graph already maintain the acyclic in the pre-state of the $\abg$. Hence $(\vnode(key_1) \wedge \vnode(key_2) \in \prees{\acadde(key_1,key_2,true)}) \wedge (\abg \text{ is Acyclic)}$.
    
\item Concurrent successful $\remv$ on $key_1$ or $key_2$ or both: 
We know that the $\lp$ in this case is immediately before the first $\lp$ of $\remv$ $\mth$. The Lemma \ref{lem:removeVT-conc} shows, if $\remv(key)$ returns true, the vertex node corresponding to that key is present in the pre-state of the $\lp$. If any of the vertices were not present, the method returns $false$. So we conclude that, $(\vnode(key_1) \wedge \vnode(key_2))$ $\in$ $\prees{\acadde(key_1,key_2,true)}$. And from the Lemma \ref{lem:acyclic}, the graph already maintain the acyclic in the pre-state of the $\abg$. Hence, $(\vnode(key_1) \wedge \vnode(key_2)) \in \prees{\acadde(key_1,key_2,true)}) \wedge (\abg \text{ is Acyclic)}$. 
\end{enumerate}
\item \textbf{\ref{lem:addET-conc-acyclic-post}}:
\end{itemize}
\end{proofsketch}


\begin{lemma}
\label{lem:addEF-conc-acyclic}
If some $\acadde(key_1,key_2)$ method returns false in $E^H$, then 
\begin{enumerate}[label=\ref{lem:addEF-conc-acyclic}.\arabic*]
\item \label{lem:addEF-conc-acyclic-pre}
At least one of the vertex nodes corresponding to those keys will not be present in the pre-state of \lp event of the method and the graph is acyclic. Formally, $\langle$ $\acadde(key_1,key_2, false) \Longrightarrow (\vnode(key_1)$ $\vee$ $\vnode(key_2)) \notin \prees{\acadde(key_1,key_2, false)}) \wedge (\abg \text{ is Acyclic })\rangle$. 
\item \label{lem:addEF-conc-acyclic-post}
At least one of the vertex nodes corresponding to those keys will not be present in the post-state of \lp event of the method and the graph is acyclic. Formally, $\langle$ $\acadde(key_1,key_2, false) \Longrightarrow (\vnode(key_1)$ $\vee$ $\vnode(key_2)) \notin \postes{\acadde(key_1,key_2, false)}) \wedge (\abg \text{ is Acyclic })\rangle$. 
\end{enumerate}
\end{lemma}

\begin{proofsketch}
\begin{itemize}
\item \textbf{\ref{lem:addEF-conc-acyclic-pre}}:
\begin{enumerate}
\item No successful concurrent $\addv$ on $key_1$ and $key_2$:
 By observing the code, we realise that in the Line \ref{lin:helploce8}/\ref{lin:helploce8.1} vertex node $\vnode(key_1)$ is not in the $S.\abgv$ because it is not reachable from $\vh$ or marked. Also, in the Line \ref{lin:helploce16}/\ref{lin:helploce16.1} vertex node $\vnode(key_2)$ $\notin$ $S.\abgv$ because it is not reachable from $\vh$ or marked. Consequently, the Line \ref{lin:loce8:16} returns $false$, if $read(v_1.marked)$ or $read(v_2.marked)$ is set depending upon the execution. So ($)\vnode(key_1)$ $\vee$ $(\vnode(key_2)$) $\notin$ $\pree{i}$. If ($\vnode(key_1)$ $\vee$ $(\vnode(key_2)$) $\in$ $\pree{i}$ and $\adde(key_1,key_2)$ checks in the Line \ref{lin:addedge:cycle} that there is a path from the $\vnode(key_2)$ to $\vnode(key_1)$, to check presence of a cycle in the graph. If cycle exists in the Line \ref{lin:status-addec14} the edge is removed and the graph maintain acyclic invariant like previous operations by the property of the Lemma \ref{lem:acyclic}. Hence, $(\vnode(key_1)$ $\vee$ $\vnode(key_2)) \notin \prees{\acadde(key_1,key_2, false)}) \wedge (\abg \text{ is Acyclic)})$
 
\item Concurrent successful $\addv$ on $key_1$ or $key_2$ or both: 
We know that the $\lp$ in this case is immediately before the first $\lp$ of $\addv$ $\mth$ on $u$ and $v$. Also from the Lemma \ref{lem:addVT-conc}, it follows that if $\addv(key)$ returns true, then the vertex node corresponding to that key is not present in the pre-state of the $\lp$.  And from the Lemma \ref{lem:acyclic}, the graph already maintain the acyclic in the pre-state of the $\abg$. Hence, $(\vnode(key_1) \vee \vnode(key_2)) \notin \prees{\acadde(key_1,key_2, false)}) \wedge (\abg \text{ is Acyclic)}$. 

\end{enumerate}
\item \textbf{\ref{lem:addEF-conc-acyclic-post}}:
\end{itemize}
\end{proofsketch}

\begin{lemma}
\label{lem:adde-pre-acyclic}

For some $\acadde(key_1,key_2)$ method the graph is acyclic in the pre-state of \lp event of the method then in the post-state of \lp event of the method of the graph is also acyclic. Formally, $\langle$ $(\prees{\acadde(key_1,key_2, true)} \text{ is acyclic}) \xRightarrow[]{\acadde(key_1,key_2, true)} \postes{\acadde(key_1,key_2, true)} \text{ is Acyclic }\rangle$. 

\end{lemma}

\begin{proofsketch}
From the Lemma \ref{lem:acyclic} after each methods operation the graph is acyclic invariant. And we know that only $\acadde$ \mth can form the cycle in the graph. Before $\adde$ in the pre-state of the $\lp$ event the graph is acyclic. After successful $\acadde(key_1,key_2)$ method from the Lemma \ref{lem:addET-conc-acyclic} the graph is also acyclic in the post-state of the $\lp$ event. Hence, if the \\ $\prees{\acadde(key_1,key_2, true)} \text{ is acyclic}$, after successful $\acadde$ $\prees{\acadde(key_1,key_2, true)} \text{ is acyclic}$.
\end{proofsketch}

\begin{lemma}
\label{lem:acyclic}
	In any execution of the reachability algorithm, all the edges of the graph with the state $added$ do not form a cycle.
\end{lemma}

\begin{proofsketch}

From the \lemref{addET-conc-acyclic}, \ref{lem:addEF-conc-acyclic} and \ref{lem:adde-pre-acyclic}.
\end{proofsketch}
%We prove by Induction on events that change the state of an edge node.

%Base step:

%Induction Hypothesis:

%Induction Step:


\subsection{Liveness: Proof Outline}
In this subsection we prove the progress guarantee of the methods of our proposed graph data structure with acyclic property. 
\begin{lemma}
	The methods $\addv$, $\remv$, $\acadde$ and $\acreme$ are deadlock-free.
\end{lemma}

\begin{proofsketch}

\noindent
The proof of the $\addv$, $\remv$, $\acadde$ and $\acreme$ methods are deadlock-free by direct argument based of the acquiring lock on both the current and predecessor nodes. The $\addv$ and $\remv$ proof are similar argument as Lemma \ref{lem:prog:add:rem}.1 and \ref{lem:prog:add:rem}.2 respectively. And the proof of $\acadde$ and $\acreme$ is given bellow. 
\begin{enumerate}
    \item $\acadde$: the $\acadde(key_1, key_2)$ method is deadlock-free because a thread always acquires lock on the $\enode$ with smaller keys first. Which means, if a thread say $T_1$ acquired a lock on a $\enode(key_2)$, it never tries to acquire a lock on a $\enode$ of the vertex $\vnode(key_1)$ with key smaller than or equal to $\enode(key_2)$. This is true because the $\acadde$ method acquires lock on the predecessor edge nodes of the vertex $\vnode(key_1)$ from the $AcyclicLocateEdge$ method and returns after releasing the locks.
    \item $\acreme$: the $\acreme(key_1, key_2)$ method is also deadlock-free, similar argument as $\acadde$.
\end{enumerate}
\end{proofsketch}


\begin{lemma}
	The methods $\conv$, $\accone$ and $PathExists$ are wait-free.
\end{lemma}

\begin{proofsketch}
\noindent The proof of the $\conv$ and $\accone$ method is similar arguments as \ref{lem:prog:con}.1 and \ref{lem:prog:con}.2 respectively. 
%And the proof the $PathExists$ is given below: \\

%\Comment{How $PathExists$ is wait-free? It is called inside \adde and both the nodes are locked.}

\end{proofsketch}


==> app-gen-graph.tex <==
\section{Sequential Specification}
\label{sec-app-seq-spec}
\noindent Given a global state $S$, we now define the notion of an abstract graph(for \fg, \lf and \wf, as \cg \& sequential are straight forward) , $\abg$ for a global state $S$ which we will use for guiding us in correctness of our \mth{s}. $\abg$ for a global state $S$ is the collection of $S.\abgv$ and $S.\abge$ as defined below:
 

\begin{table*}[!ht]
\captionsetup{font=scriptsize}
 \centering
  \captionof{table}{Sequential Specification of the Graph Data-Structure } \label{tab:seq-spe} 
  \scriptsize
\begin{tabular}{ |m{3cm}|m{1cm}|m{4.5cm}|m{4.5cm}| } 

\hline
  \textbf{Method} & \textbf{Return Value} & \textbf{Pre-state}($S$: global state)  & \textbf{Post-state}( $S'$: future state of $S$ such that $S \sqsubset S'$)  \\ 
  
  \hline
	$\addv (u)$  & $true$ &$ S: \langle u \notin S.\abgv \rangle $ &$ S':\langle u \in S'.\abgv \rangle$	 \\
\hline 
	$\addv (u)$  & $false$ & Never the case	 &Never the case 	 \\
\hline 
	$\remv (u)$  & $true$ &$ S: \langle u \in S.\abgv \rangle$ &$ S':\langle u \notin S'.\abgv \rangle$	 \\
	\hline 
$\remv (u)$  & $false$ &$ S: \langle u \notin S.\abgv \rangle$ &Same as pre-state \\%$\forall S:(u \notin S.\abgv)$	 \\
	\hline 
	$\adde (u, v)$  & $true$ &$ S: \langle u,v \in S.\abgv \wedge  ((u,v) \in S.\abge \vee (u,v) \notin S.\abge ) \rangle$ & $ S':\langle (u,v \in S'.\abgv \wedge (u,v) \in S'.\abge \rangle$	 \\
	\hline 
	$\adde(u, v)$  & $false$ &$ S: \langle  u \notin S.\abgv \vee v \notin S.\abgv \rangle$ &Same as pre-state \\%$\forall S: ((u,v) \notin S.S(E).AbG)  \vee (u \notin S.\abgv) \vee (v \notin S.\abgv)$ 
	\hline 
	$\reme(u, v)$  & $true$ &$ S: \langle u,v \in S.\abgv \wedge  ((u,v) \in S.\abge) \vee (u,v) \notin S.\abge ) \rangle$ &$ S':\langle u,v \in S'.\abgv) \wedge (u,v) \notin S'.\abge \rangle$	 \\	
	\hline 
	$\reme(u, v)$  & $false$ &$ S: \langle u\notin S.\abgv \vee v\notin S.\abgv \rangle $ & Same as pre-state \\ %$\forall S:((u\notin S.\abgv) \vee (v\notin S.\abgv)) \vee ((u,v) \notin S.S(E).AbG)$	 \\	
	\hline 
	$\conv(u)$  & $true$ &$ S: \langle u \in S.\abgv \rangle$ &Same as pre-state \\%$\forall S:(u \in S.\abgv)$	 \\
	\hline 
	$\conv(u)$  & $false$ &$ S: \langle u \notin S.\abgv \rangle$ &Same as pre-state \\ %\forall S:(u \notin S.\abgv)$	 \\
	\hline 
	$\cone(u, v)$  & $true$ &$ S: \langle u,v \in S.\abgv \wedge  (u,v) \in S.\abge  \rangle$ & Same as pre-state \\%$\forall S:(u,v \in S.\abgv) \wedge (v \in S.S(E).AbG)$	 \\
	\hline 
	$\cone(u, v)$  & $false$ &$ S: \langle u\notin S.\abgv \vee v\notin S.\abgv \vee  (u,v) \notin S.\abge \rangle$ &same as pre-state	 \\
 
\hline

\end{tabular}
%\vspace{-5mm}
\end{table*}
 \begin{definition}
\label{def:abgV}
	$S.\abgv \equiv \{v | (v \in \vnodes{S}) \land (S.\vh \rightarrow^* S.v) \land (\neg S.v.marked)\}$.
\end{definition}

\noindent This definition of \abgv captures the set of all vertices of $\abg$ for the global state $S$. It consists of all the \vnode{s} that are reachable from $S.\vh$ and are not marked for deletion. 

\begin{definition}
\label{def:abgE}
	$S.\abge \equiv \{e | (e \in S.enodes) \land ((u, v) \subseteq S.\abgv) \land \\ (S.u.\eh \rightarrow^* S.e) \land (\neg S.e.marked) \land (S.e.val = S.v.val)\}$.
\end{definition}

\noindent This definition of $\abge$ captures the set of all edges of $\abg$ for the global state $S$. Informally it consists of all the $\enode$s that connects two $\vnode$s $u$, $v$ with the edge going form $u$ to $v$. 

==> app-model.tex <==
\section{System Model \& Preliminaries}
\label{sec:app-model}
\vspace{-1mm}
\noindent \textbf{Events.} We assume that the threads execute atomic \emph{events} which are (1) read, write on shared/local memory objects; (2) \mth invocations or \emph{\inv} event \& responses or \emph{\rsp} event on higher level shared-memory objects. %(2) acquire \& release on lock objects;

%\textbf{Events.} We assume that the threads execute atomic \emph{events} . Similar to Lev{-}Ari et. al.'s work, \cite{Lev-Aridisc2015, Lev-Aridisc2014} we assume that these events by different threads are (1) read, write on shared/local memory objects; (2) \mth invocations or \emph{\inv} event \& responses or \emph{\rsp} event on higher level shared-memory objects. %(2) acquire \& release on lock objects; 

\vspace{1mm}
\noindent
\textbf{Global States, Execution and Histories.} We define the \emph{global state} or \emph{state} of the system as the collection of local and shared variables across all the threads in the system. The system starts with an initial global state. We assume that all the events executed by different threads are totally ordered. Each event changes possibly the global state of the system leading to a new global state. 

The events \emph{read, write} on shared/local memory objects changes the global state. The events $\inv$ event \& $\rsp$ event on higher level shared-memory objects do not change the contents of the global state. Although we denote the resulting state with a new label. 

We denote an \emph{execution} of a concurrent threads as a finite sequence of totally ordered atomic events. We formally denote an execution $E$ as the tuple $\langle evts, <_E \rangle$, where $\eevts{E}$ denotes the set of all events of $E$ and $<_E$ is the total order among these events. A \emph{history} corresponding to an execution consists only of \mth \inv and \rsp events (in other words, a history views the \mth{s} as black boxes without going inside the internals). Similar to an execution, a history $H$ can be formally denoted as $\langle evts, <_H \rangle$ where $evts$ are of type $\inv$ \& $\rsp$ and $<_H$ defines a total order among these events. 

With this definition, it can be seen that a history uniquely characterizes an execution and vice-versa. Thus we use these terms interchangeably in our discussion. For a history $H$, we denote the corresponding execution as $E^H$. %Given an execution $E$, we denote the corresponding history $H$ as $\hst{E}$. Similarly, for a history $H$, we denote the corresponding execution as $\exec{H}$. 

We relate executions (histories) with global states. An execution takes the system through a series of global states with each event of the execution stating from the initial state takes the global state from one to the next. We associate the state of an execution (or history) to be global state after the last event of the execution. We denote this final global state $S$ of an execution E as $S = \state{E}$ (or $\state{H}$). 

We refer to the set of all the global states that a system goes through in the course of an execution as $\alls{E}$ (or $\alls{H}$). It can be seen that for $E$, $\state{E} \in \alls{E}$. \figref{exec/hist} show an execution and the corresponding history. In the figure the curve line is an event, the vertical line is a state. The open([) \& close(]) square bracket are the separator and it has no meaning in the figure.
\vspace{-1mm}

\begin{figure}[H]
\captionsetup{font=scriptsize}
	\centerline{\scalebox{0.525}{\input{figs/ExeHist.pdf_t}}}
	\caption{Figure (a) depicts a Concurrent Execution $E^H$ comprising of multiple events. $E.state$ denotes the global state after the last event of the execution. Figure (b) depicts the corresponding concurrent history $H$ consisting only of $inv$ and $resp$ events. $H.state$ denotes the global state after the last event in the history.}
	\label{fig:exec/hist}
\end{figure}
\vspace{-2mm}
Given an event $e$ of an execution $E$, we denote global state just before the $e$ as the pre-state of $e$ and denote it as $\pres{e}$. Similarly, we denote the state immediately after $e$ as the the post-state of $e$ or $\posts{e}$. Thus if an event $e$ is in $\eevts{E}$ then both $\pres{e}$ and $\posts{e}$ are in $\alls{E}$.

The notion of pre \& post states can be extended to \mth{s} as well. We denote the pre-state of a \mth $m$ or $\pres{m}$ as the global state just before the invocation event of $m$ whereas the post-state of $m$ or $\pres{m}$ as the global state just after the return event of $m$. 

\vspace{1mm}
\noindent
\textbf{Notations on Histories.} We now define a few notations on histories which can be extended to the corresponding executions. We say two histories $H1$ and $H2$ are \emph{equivalent} if the set of events in $H1$ are the same as $H2$, i.e., $\eevts{H1} = \eevts{H2}$ and denote it as $H1 \approx H2$. We say history $H1$ is a \emph{\subh} of $H2$ if all the events of $H1$ are also in $H2$ in the same order, i.e., $\langle (\eevts{H1} \subseteq \eevts{H2}) \land (<_{H1} \subseteq <_{H2}) \rangle$. 

Let a thread $T_i$ invoke some \mth{s} on a few shared memory objects in a history $H$ and $o$ be a shared memory object whose \mth{s} have been invoked by threads in $H$. Using the notation of \cite{HerlWing:1990:TPLS}, we denote $H|T_i$ to be the \subh all the events of $T_i$ in $H$. Similarly, we denote $H|o$ to be the \subh all the events involving $o$.

We say that a \rsp event \emph{matches} an \inv event in an execution (as the name suggests) if the both \rsp and \inv events are on the same \mth of the object, have been invoked by the same thread and the \rsp event follows \inv event in the execution. 

We assume that a history $H$ as \emph{well-formed} if a thread $T_i$ does not invoke a \mth on a shared object until it obtains the matching response for the previous invocation. We assume that all the executions \& histories considered in this paper are well-formed. We denote an \inv event as \emph{pending} if it does not have a matching \rsp event in the execution. Note that since an execution is well-formed, there can be at most only one pending invocation for each thread. 

We say a history $H$ is \emph{complete} if for every \mth \inv event there is a matching \rsp event. The history $H$ is said to be \emph{sequential} if every \inv event, except possibly the last, is immediately followed by the matching \rsp event. Note that a complete history is not sequential and the vice-versa. It can be seen that in a well-formed history $H$, for every thread $T_i$, we have that $H|T_i$ is sequential. \figref{seqhist} shows a sequential history. 

\begin{figure}[th]
\captionsetup{font=scriptsize}
	\centerline{\scalebox{0.45}{\input{figs/seqspec.pdf_t}}}
	\caption{An illustration of a Sequential history $E^S$.}
	\label{fig:seqhist}
\end{figure}

%\vspace{-1mm}
\noindent
\textbf{Sequential Specification.} 
%If $e_{i+1}$ is \inv/\rsp event then $S_i$ = $S_{i+1}$
We next discuss about \emph{\sspec} \cite{HerlWing:1990:TPLS} of shared memory objects. The \sspec of a shared memory object $o$ is defined as the set of (all possible) sequential histories involving the \mth{s} of $o$. Since all the histories in the \sspec of $o$ are sequential, this set captures the behavior of $o$ under sequential execution which is believed to be correct. A sequential history $\mathcal{S}$ is said to be \emph{\legal} if for every shared memory object $o$ whose \mth is invoked in $S$, $\mathcal{S}|o$ is in the \sspec of $o$. 

\vspace{1mm}
\noindent
\textbf{Safety:} A \emph{safety} property is defined over histories (and the corresponding executions) of shared objects and generally states which executions of the shared objects are acceptable to any application. The safety property that we consider is \emph{linearizability} \cite{HerlWing:1990:TPLS}. A history $H$ is said to be linearizable if (1) there exists a completion $\overline{H}$ of $H$ in which some pending \inv events are completed with a matching response and some other pending \inv events are discarded; (2) there exists a sequential history $\mathcal{S}$ such that $\mathcal{S}$ is equivalent to $\overline{H}$; (3) $\mathcal{S}$ is legal.

Another way to say that history $H$ is linearizable if it is possible to assign an atomic event as a \emph{linearization point} (\emph{\lp}) inside the execution interval of each \mth such that the result of each of these \mth{s} is the same as it would be in a sequential history in which the \mth{s} are ordered by their \lp{s} \cite{MauriceNir}. 

A concurrent object is linearizable if all the histories generated by it are linearizable.  We prove the linearizability of a concurrent history by defining a \lp{s} for each method. The \lp of a \mth implies that the method appears to take effect instantly at its \lp. %, and the behavior of the \mth at that instant is exactly same as defined by the sequential specification. 

%A concurrent object is linearizable if all the histories generated by it are linearizable.  We prove the linearizability of a concurrent history by defining a \textit{linearization point} or \emph{\lp} for each method in the execution at some instant between invocation and response event. This means that each method appears to occur instantly at its \lp, and the behavior of the \mth at that instant is exactly same as defined by the sequential specification. 
\ignore{
\vspace{1mm}
\noindent
\textbf{Progress:} The \emph{progress} properties specifies when a thread invoking \mth{s} on shared objects completes in presence of other concurrent threads. Some progress conditions used in this paper are mentioned here which are based on the definitions in Herlihy \& Shavit \cite{opodis_Herlihy}. The progress condition of a method in concurrent object is defined as: (1) Blocking: In this, an unexpected delay by any thread (say, one holding a lock) can prevent other threads from making progress. (2) Deadlock-Free: This is a \textbf{blocking} condition which ensures that \textbf{some} thread (among other threads in the system) waiting to get a response to a \mth invocation will eventually receive it. (3) Wait-Free: This is a \textbf{non-blocking} condition which ensures that \textbf{every} thread trying to get a response to a \mth, eventually receives it.
}
\ignore{
\textbf{Progress:} The \emph{progress} properties specifies when a thread invoking \mth{s} on shared objects completes in presence of other concurrent threads. Some progress conditions used in this paper are mentioned here which are based on the definitions in Herlihy \& Shavit \cite{opodis_Herlihy}. The progress condition of a method in concurrent object is defined as: 
\begin{enumerate}
\item  \textbf{Blocking}: In this, an unexpected delay by any thread (say, one holding a lock) can prevent other threads from making progress. 
\item \textbf{Deadlock-Free}: This is a \textbf{blocking} condition which ensures that \textbf{some} thread (among other threads in the system) waiting to get a response to a \mth invocation will eventually receive it. 

\item \textbf{Starvation-Free}: This is a \textbf{blocking} condition which ensures that \textbf{every} thread trying to get a response to a \mth, eventually receives it. 
\item \textbf{Non-Blocking}: In this, a failure or suspension of a thread cannot prevent some operation of another thread from making progress.

\item \textbf{Lock-Free}: This is a \textbf{non-blocking} condition which ensures that \textbf{some} thread waiting to get a response to a \mth (among multiple other threads), eventually receives it. 
\item \textbf{Wait-Free}: This is a \textbf{non-blocking} condition which ensures that \textbf{every} thread trying to get a response to a \mth, eventually receives it.
 
\end{enumerate}
}
\noindent It can be seen that wait-free \mth{s} are desirable since they can complete regardless of the execution of other concurrent \mth{s}. On the other hand, deadlock-free \mth{s} are system (or underlying scheduler) dependent progress condition since they involve blocking. It ensures that among multiple threads in the system, at least one of them will make progress.\\

\noindent The update \mth{s} exported by the graph data-structure discussed in this paper are deadlock-free and the contains \mth{s} are wait-free.

%The \emph{progress} properties specifies when a thread invoking \mth{s} on shared objects completes in presence of other concurrent threads. Some progress conditions used in this paper are mentioned here which are based on the definitions in Herlihy \& Shavit \cite{opodis_Herlihy}. The progress condition of a method in concurrent object is defined as: (1) Blocking: In this, an arbitrary and unexpected delay by any thread (say, one holding a lock) can prevent other threads from making progress. (2) Deadlock-Free: This is a \textbf{blocking} condition which ensures that \textbf{some} thread waiting to get a response to a \mth (among multiple other threads), eventually receives it. (3) Starvation-Free: This is a \textbf{blocking} condition which ensures that \textbf{every} thread trying to get a response to a \mth, eventually receives it. (4) Lock-Free: This is a \textbf{non-blocking} condition which ensures that \textbf{some} thread waiting to get a response to a \mth (among multiple other threads), eventually receives it. (5) Wait-Free: This is a \textbf{non-blocking} condition which ensures that \textbf{every} thread trying to get a response to a \mth, eventually receives it.
\ignore{	
\begin{itemize}
\item Blocking: In this, an arbitrary and unexpected delay by any thread (say, one holding a lock) can prevent other threads from making progress.
\item Deadlock-Free: This is a \textbf{blocking} condition which ensures that \textbf{some} thread waiting to get a response to a \mth (among multiple other threads), eventually receives it.
\item Starvation-Free: This is a \textbf{blocking} condition which ensures that \textbf{every} thread trying to get a response to a \mth, eventually receives it.
\item Lock-Free: This is a \textbf{non-blocking} condition which ensures that \textbf{some} thread waiting to get a response to a \mth (among multiple other threads), eventually receives it.
\item Wait-Free: This is a \textbf{non-blocking} condition which ensures that \textbf{every} thread trying to get a response to a \mth, eventually receives it.
\end{itemize}

}

\ignore {
\subsection{Related Work}
\noindent There have been a lot of works on \textit{Dynamic graph} on different graph algorithms. But there are very few papers on concurrent graph, one of the recent work on concurrent graph objects is by Kallimanis and Eleni \cite{Kallimanis}. They talk about how their concurrent graph model supports concurrent operations; adding vertices or edges, deleting vertices or edges and dynamic traversal. They represent dynamic graph in the form of adjacency matrix with fixed number of vertices and it allows only the addition, and deletion of edges and the modification of edge weights. Also there has been a lot of work on incremental cycle detection \cite{Bernhard, Pearce} in the sequential environment. A nice classical result of graph theory is that, a directed graph is cycle-free if and only if it has a topological order\cite{Cormen}, or rather if the strong components of a directed graph can be ordered topologically. For static directed graphs, there are two $O(m)$-time algorithms to find a cycle or a topological order and depth-first search \cite{Kahn,Knuth}(the reverse post-order defined by such a search is a topological order if the graph is acyclic). Depth-first search extends to find the strong components in a directed graph and a topological order of them in $O(m)$  \cite{Knuth}.

The problem of cycle detection has also been well explored in distributed systems. The problem was proposed by Chandy, et al. \cite{Chandy} and it has also been explored by \cite{Ambroise,Knapp}. They use local \textit{wait-for-graphs}(WFG)\cite{Galvin} to detect cycle in the local copy and then probe to confirm the existence of cycle in the global WFG.

The snapshot problem was discussed by Guerraoui and Ruppert \cite{Rachid}. Snapshots will not be consistent if we read one value at a time \cite{Faith}. The problem lies in the fact that the first value read might have become outdated by the time later values are read. Therefore there is a need of an atomic implementation of snapshot \cite{Afek}. Snapshots have been well explored even in distributed systems \cite{Ranganath}.  

To prove a concurrent data-structure correct, the linearizability was first defined by Herlihy and Wing \cite{Maurice} and then it was well explored formally by \cite{Peter-podc2010,Vafeiadis-ppopp2006, Lev-Aridisc2015, Lev-Aridisc2014}. 
}


==> related-work.tex <==
\section{Related Works}
\label{sec:related-work}

